Causative Cyberattacks on Online Learning-based Automated Demand Response Systems

Power utilities are adopting Automated Demand Response (ADR) to replace the costly fuel-fired generators and to preempt congestion during peak electricity demand. Similarly, third-party Demand Response (DR) aggregators are leveraging controllable small-scale electrical loads to provide on-demand grid support services to the utilities. Some aggregators and utilities have started employing Artificial Intelligence (AI) to learn the energy usage patterns of electricity consumers and use this knowledge to design optimal DR incentives. Such AI frameworks use open communication channels between the utility/aggregator and the DR customers, which are vulnerable to \textit{causative} data integrity cyberattacks. This paper explores vulnerabilities of AI-based DR learning and designs a data-driven attack strategy informed by DR data collected from the New York University (NYU) campus buildings. The case study demonstrates the feasibility and effects of maliciously tampering with (i) real-time DR incentives, (ii) DR event data sent to DR customers, and (iii) responses of DR customers to the DR incentives.

==> Updated_Source_File_for_Line_Number_280_to_310.tex <==
\subsubsection{Online Exploration of the Utility Function of DR Customers}
\label{sec:learn_utility_function_DR}
In the set up of Fig.~\ref{fig:attack}, the utility or  aggregator can  sequentially record broadcasted DR incentives and reductions in power consumption  of the DR customers in response to the incentives. Using this recorded  data, $\mathcal{H}_t =\{\lambda_{\tau},$ $x_{i,\tau}\},~\forall i \in \mathcal{N},~\forall \tau \in \mathcal{T}$, where $\mathcal{{N}} =\{1,\ldots, N\}$, $\mathcal{T} =\{1,\ldots, t-1\}$, $|\mathcal{T}|=T$, and $|\mathcal{N}|=N$, the utility or aggregator estimates $\boldsymbol{\beta}_{i,t}$ by minimizing the Mean Squared Error (MSE) of the expected response of DR customers given by Eq.~\eqref{eq:x_DR_opt}. This objective can be parameterized by the empirical loss function: 
\begin{subequations}
\label{eq:MSE}
\begin{align}
   \label{eq:loss}
    L_{i,t}((\lambda,x);\boldsymbol{\beta})= \frac{1}{2T}\sum_{\tau=1}^{T}(x_{i,\tau}-\beta_{1,i,\tau}\lambda_{\tau} -\beta_{0,i,\tau})^2 .
\end{align}
The first order optimality condition of $L((\lambda,x); \boldsymbol{\beta})$ over $\boldsymbol{\beta}_{i,t}$ is expressed as:
\begin{align}
\label{eq:partial_R1}
   \frac{\partial L_{i,t}}{\partial \beta_{1,i,t}} &=\frac{1}{T}\sum_{\tau=1}^{T} (x_{i,\tau}\lambda_{\tau}-\beta_{1,i,\tau}\lambda_{\tau}^2-\beta_{0,i,\tau}\lambda_{\tau}) =0, \\
   \label{eq:partial_R2}
   \frac{\partial L_{i,t}}{\partial \beta_{0, i, t}} &=\frac{1}{T}\sum_{\tau=1}^{T} (x_{i,\tau}-\beta_{1,i,\tau}\lambda_{\tau}-\beta_{0,i,\tau}) =0.
\end{align}
Solving Eqs.~\eqref{eq:partial_R1} and \eqref{eq:partial_R2} and setting $ \frac{1}{T}\sum_{\tau=1}^{T} x_{i,\tau} =\hat{x}_{i,t}$  and $ \frac{1}{T}\sum_{\tau=1}^{T} \lambda_{\tau} =\hat{\lambda}_{t}$, it follows:
\allowdisplaybreaks
\begin{align}
\label{eq:beta1}
    \beta_{1,i,t} &=\frac{\frac{1}{T}\sum_{\tau=1}^{T}x_{i,\tau}\lambda_{\tau} -\hat{x}_{i,t}\hat{\lambda}_{t}}{\frac{1}{T}\sum_{\tau=1}^{T}\lambda^2_{\tau}-\hat{\lambda}^2_{t}},\\
    \label{eq:beta0}
    \beta_{0,i,t} &=\hat {x}_{i,t}-\beta_{1,i,t}\hat{\lambda}_{t}.
\end{align}
Since set $\mathcal{H}_t$  is updated at every DR event at time $t$, Eqs.~\eqref{eq:beta1} and \eqref{eq:beta0}  use \textit{streaming} historical data to estimate $\boldsymbol{\beta}_{i,t}$. This is computationally unattractive for all DR customers over time due to the addition of new data points $\{x_{i,t}, \lambda_t\}$  at each DR event at time $t$. To overcome the computational complexity, the utility or aggregator can use the online gradient descent to update $\boldsymbol{\beta}$ for a DR event at time $t+1$ as:
\begin{align}
 \label{eq:ogd}
     \boldsymbol{\beta}_{i,t+1} = \boldsymbol{\beta}_{i,t}- {\eta_l}(\boldsymbol{\beta}^{\top}_{i,t}\boldsymbol{\lambda}_{t} -x_{i,t})\lambda_{t},
\end{align}
\end{subequations}
where ${\eta_l}$ is a user-defined model learning rate and vector $\boldsymbol{\lambda}_{t} = [1 ~ \lambda_{t}]^{\top}$. In the setting of Eq.~\eqref{eq:ogd}, $\boldsymbol{\beta}$ obtained in Eqs.~\eqref{eq:beta1} and \eqref{eq:beta0} can be realized as $\boldsymbol{\beta}_{i,t}$, which is updated at time $t+1$ to $\boldsymbol{\beta}_{i,t+1}$ based on the new sample set $\{x_{i,t}, \lambda_t\}$ of the DR event at time $t$.
